Jack The Rippler: Arbitrage on the Decentralized Exchange of the XRP Ledger

The XRP Ledger (XRPL) is a peer-to-peer cryptographic ledger. It features a decentralized exchange (DEX) where network participants can issue and trade user-defined digital assets and currencies. We present Jack the Rippler, a bot that identifies and exploits arbitrage opportunities on the XRPL DEX. We describe Jack's arbitrage process and discuss risks associated with using arbitrage bots.

==> exhibits/nodedist.tex <==
\begin{table}[h]
\footnotesize
\begin{subtable}[h]{0.495\columnwidth}
\centering
\begin{tabular}{ c|c }
\toprule
Countries & Nodes \\
 \midrule
 United States & 54\% \\ 
 Japan & 13\% \\ 
 South Korea & 7\% \\ 
 Others & 26\% \\ 
 \bottomrule
 \end{tabular}
 \caption{Node distribution} 
 \label{table:nodedist} 
\end{subtable}
\begin{subtable}[h]{0.495\columnwidth}
\centering
\begin{tabular}{ c|c }
\toprule
Countries & UNL Validators \\
 \midrule
 United States & 65\% \\ 
 Germany & 7\% \\ 
 Singapore & 5\% \\ 
 Others & 23\% \\ 
 \bottomrule
 \end{tabular}
 \caption{UNL nodes distribution} 
\label{table:unldist} 
\end{subtable}
\caption{UNL nodes distribution} 
\end{table}
